Distributed Sketching Methods for Privacy Preserving Regression

In this work, we study distributed sketching methods for large scale regression problems. We leverage multiple randomized sketches for reducing the problem dimensions as well as preserving privacy and improving straggler resilience in asynchronous distributed systems. We derive novel approximation guarantees for classical sketching methods and analyze the accuracy of parameter averaging for distributed sketches. We consider random matrices including Gaussian, randomized Hadamard, uniform sampling and leverage score sampling in the distributed setting. Moreover, we propose a hybrid approach combining sampling and fast random projections for better computational efficiency. We illustrate the performance of distributed sketches in a serverless computing platform with large scale experiments.

==> acknowledgements.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> summary.tex <==
% \section{Summary of Results}

% Table \ref{result_summary_table} gives a summary of the results for averaged least squares.

% \begin{table}%*}%[t]
% \centering
% \caption{Summary of bounds for bias and variance for the single sketch estimator $\hat{x}_k$. Gaus: Gaussian, Unif: Uniform sampling, Lvrg: Leverage score sampling.}
% \label{result_summary_table}
%  \begin{tabular}{||c |c c c||} 
%  \hline
%   & Squared norm of bias & High prob. bound on  &  \\ 
%  Sketch & $\frac{\| \Exs [A\hat{x}_k]-Ax^* \|_2^2 }{f(x^*)} \leq $ & variance $\frac{||A\hat{x}_k-Ax^*||_2^2}{f(x^*)} \leq $ & $m \geq $  \\
%  [0.5ex] 
%  \hline\hline
%  Gaus & $0$ & $\frac{d}{m-d-1}$ & $d+1$ \\
%  \hline
%  ROS & $4\epsilon\frac{d}{m}$ & $\mathcal{O}\left(\frac{d\log d}{m} \right) $ &   \\ 
%  \hline
%  Unif & $ \frac{4\epsilon n}{m} \frac{n-m}{n-1}\,  \max_i \|\tilde{u}_i \|_2^2$ & $\mathcal{O}\left(\frac{n\log d}{m} \max_i ||\tilde{u}_i||_2^2 \right) $ &   \\ 
%  \hline
%  Lvrg & $4\epsilon \frac{d}{m} $ & $\mathcal{O}\left(\frac{d\log d}{m} \right) $ &   \\ 
%  \hline
% \end{tabular}
% \end{table}%*}


\begin{table}
\centering
\caption{Summary of bias bounds for the single sketch estimator $\hat{x}_k$. (Gaus: Gaussian, Uniform: Uniform sampling, Lvrg: Leverage score sampling.)}
\label{result_summary_table}
 \begin{tabular}{||c |c c c c||} 
 \hline
 Bias & Gaus & ROS & Uniform & Lvrg \\
 [0.5ex] 
 \hline\hline
 $\frac{\| \Exs [A\hat{x}_k]-Ax^* \|_2^2 }{f(x^*)} \leq $ & $0$ & $4\epsilon\frac{d}{m}$ & $ \frac{4\epsilon n}{m} \frac{n-m}{n-1}  \max_i \|\tilde{u}_i \|_2^2$ & $4\epsilon \frac{d}{m}$ \\
 \hline
\end{tabular}
\end{table}



% Table \ref{all_methods_table} gives a summary of the results for averaged least squares.


% \begin{table*}[t]
% \centering
% \caption{Comparison against other algorithms. The big-$\mathcal{O}$ notation concealed for some of entries of the table. The abbreviations used in the table stand for: Gaus: Gaussian, Unif: uniform, Sync: synchronous, Async: asynchronous, Comm: communication, Dist: distributed.}
% \label{all_methods_table}
%  \begin{tabular}{||c |c| c c c c c||} 
%  \hline
%  Algorithm & Sketch & Complexity  & Number of & Comm. & Accuracy & Sync/ \\ 
%   & type & (per worker) & iterations  & load &  & Async \\
%  [0.5ex] 
%  \hline\hline
%  Dist. GD &  &  &  &  &  & \\
%  \hline
%  Hogwild &  &  &  &  &  & \\
%  \hline
%  Alg. \ref{distrib_avg_alg} & Gaus &  & $1$ & $qd$ &  & Async \\
%  \hline
%  Alg. \ref{distrib_avg_alg} & SRHT &  & $1$ & $qd$ &  & Async \\
%  \hline
%  Dist. right sketch, Alg. \ref{dist_rightsketch_alg} & Gaus &  & $1$ & $qd$ &  & Async \\
%  \hline
% \end{tabular}
% \end{table*}


